RuNNE-2022 Shared Task: Recognizing Nested Named Entities

The RuNNE Shared Task approaches the problem of nested named entity recognition. The annotation schema is designed in such a way, that an entity may partially overlap or even be nested into another entity. This way, the named entity "The Yermolova Theatre" of type "organization" houses another entity "Yermolova" of type "person". We adopt the Russian NEREL dataset for the RuNNE Shared Task. NEREL comprises news texts written in the Russian language and collected from the Wikinews portal. The annotation schema includes 29 entity types. The nestedness of named entities in NEREL reaches up to six levels. The RuNNE Shared Task explores two setups. (i) In the general setup all entities occur more or less with the same frequency. (ii) In the few-shot setup the majority of entity types occur often in the training set. However, some of the entity types are have lower frequency, being thus challenging to recognize. In the test set the frequency of all entity types is even. This paper reports on the results of the RuNNE Shared Task. Overall the shared task has received 156 submissions from nine teams. Half of the submissions outperform a straightforward BERT-based baseline in both setups. This paper overviews the shared task setup and discusses the submitted systems, discovering meaning insights for the problem of nested NER. The links to the evaluation platform and the data from the shared task are available in our github repository: https://github.com/dialogue-evaluation/RuNNE.

==> tables/table_entities.tex <==
\subsection{Detailed comparison of systems} \label{subsection:analysis}
We have compared solutions of participant systems in two aspects. First, we compare errors in entity type annotations given a span of a named entity was correctly detected. Second, we calculate pairwise agreements of systems' answers, again only for the annotation that have exact match of spans. Both evaluations are done on the test set. In Table \ref{table:entity_mismatch} we provide top entities for which systems give wrong entity type prediction. We found that around a half of errors come from six entity types: \textsc{organization, country, work\_of\_art, state\_or\_province, event}, and \textsc{location}. The most common mismatches are the following (correct entity is on the left of the \textsc{`->'} sign): 
\begin{itemize}
\item \textsc{organization -> facility / product / city}, 
\item \textsc{country -> nationality / organization}, 
\item \textsc{work\_of\_art -> organization / law / event}, 
\item \textsc{state\_or\_province -> city / country / location}, 
\item \textsc{event -> organization / crime / disease}, 
\item \textsc{location -> state\_or\_province / city/ country}.
\end{itemize}



To assess pairwise agreements between systems, we build lists of spans that have exactly matching boundaries, but may have different type annotations. Then we calculate Cohen's $\kappa$ for each pair of systems (Fig. \ref{fig:heatmap_triangle_aggr}). Depending on a pair of systems, the number of matching spans varies between 1,294 and 5,826. Due to this difference, values in the Figure \ref{fig:heatmap_triangle_aggr} slightly deviate from the ranking of the systems. Three teams (\textbf{svetlan}, \textbf{botbot} and \textbf{Stud2022}) have highest agreement. Also these three teams have the highest agreement with the \textbf{pullenti} team.

\begin{table}[!h]
    \centering
    \small
    
    \begin{tabular}{lrrrrrrrrrrrr}
    \toprule
Entity Type & baseln. & pullenti & abros. & MSU.& svetlan & LIORI & botbot & SibNN & Stud2022 & mojesty\\ 
    \midrule


\textsc{organization} & 23 & 21 & 28 & 21 & 20 & 18 & 17 & 29 & 14 & 24\\ 
\textsc{country} & 8 & 36 & 19 & 12 & 27 & 21 & 15 & 12 & 19 & 34\\ 
\textsc{work\_of\_art} & 22 & 3 & 20 & 16 & 1 & 16 & 2 & 24 & 1 & 23\\ 
\textsc{state\_or\_prov.} & 11 & 6 & 21 & 9 & 5 & 18 & 4 & 18 & 4 & 29\\ 
\textsc{event} & 10 & 9 & 17 & 8 & 20 & 7 & 5 & 13 & 15 & 8\\ 
\textsc{location} & 9 & 8 & 12 & 8 & 6 & 18 & 8 & 5 & 6 & 10\\ 
\textsc{facility} & 6 & 9 & 11 & 11 & 5 & 7 & 2 & 10 & 3 & 10\\ 
\textsc{nationality} & 8 & 2 & 6 & 7 & 8 & 10 & 2 & 9 & 5 & 7\\ 
\textsc{product} & 9 & 1 & 5 & 6 & - & 5 & 1 & 17 & - & 7\\ 
\textsc{city} & 6 & 5 & 7 & 5 & 6 & 9 & 3 & 5 & 3 & 11\\ 
\textsc{person} & 12 & 2 & 11 & 4 & 5 & 7 & 1 & 6 & 2 & 8\\ 
\textsc{family} & 9 & - & 10 & 6 & 2 & 7 & 1 & 8 & 1 & 7\\ 
\textsc{district} & 7 & 2 & 4 & 3 & 1 & 10 & 1 & 6 & 1 & 5\\ 
\textsc{award} & 8 & 1 & 9 & 3 & 2 & 3 & 1 & 4 & 1 & 5\\ 
\textsc{disease} & 2 & 3 & 1 & 3 & 5 & 3 & 2 & 6 & 4 & 7\\ 
\textsc{profession} & 5 & 1 & 5 & 5 & 1 & 3 & - & 5 & 1 & 6\\ 
% NUMBER & 1 & 3 & 3 & 2 & 2 & 6 & 2 & 2 & 1 & 5\\ 
% DATE & 3 & 1 & 2 & 1 & 5 & 2 & - & 2 & 6 & 1\\ 
% RELIGION & 1 & - & 5 & - & - & 1 & - & - & - & 3\\ 
% LANGUAGE & 2 & 2 & 3 & 2 & 2 & 2 & - & 2 & 1 & 4\\ 
% MONEY & 2 & - & 3 & 1 & - & - & - & 1 & - & 4\\ 
% ORDINAL & 2 & 2 & 1 & 1 & 2 & 6 & 1 & 1 & 1 & 2\\ 
% IDEOLOGY & 2 & 1 & 3 & 1 & 1 & 1 & - & - & - & 4\\ 
% TIME & - & - & 2 & - & 1 & 1 & - & 4 & 1 & 2\\ 
% PENALTY & 1 & 1 & 1 & 2 & 1 & 5 & 1 & 1 & 1 & 3\\ 
% AGE & 1 & - & 2 & 1 & - & 3 & - & 1 & - & 2\\ 
% CRIME & 2 & 3 & - & 1 & - & 1 & 1 & - & - & 1\\ 
% LAW & 1 & 1 & 2 & 2 & 1 & 2 & - & 2 & 1 & 1\\ 
% PERCENT & - & - & 1 & - & - & - & - & - & - & -


% old data:
% ORGANIZATION & 23 & 21 & 28 & 21 & 20 & 18 & 17 & 29 & 14 & 24\\ 
% COUNTRY & 8 & 36 & 19 & 12 & 27 & 21 & 15 & 12 & 19 & 34\\ 
% WORK\_OF\_ART & 22 & 3 & 20 & 16 & 1 & 16 & 2 & 24 & 1 & 23\\ 
% STATE\_OR\_PROV. & 11 & 6 & 21 & 9 & 5 & 18 & 4 & 18 & 4 & 29\\ 
% EVENT & 10 & 9 & 17 & 8 & 20 & 7 & 5 & 13 & 15 & 8\\ 
% LOCATION & 9 & 8 & 12 & 8 & 6 & 18 & 8 & 5 & 6 & 10\\ 
% FACILITY & 6 & 9 & 11 & 11 & 5 & 7 & 2 & 10 & 3 & 10\\ 
% NATIONALITY & 8 & 2 & 6 & 7 & 8 & 10 & 2 & 9 & 5 & 7\\ 
% PRODUCT & 9 & 1 & 5 & 6 & - & 5 & 1 & 17 & - & 7\\ 
% CITY & 6 & 5 & 7 & 5 & 6 & 9 & 3 & 5 & 3 & 11\\ 
% PERSON & 12 & 2 & 11 & 4 & 5 & 7 & 1 & 6 & 2 & 8\\ 
% FAMILY & 9 & - & 10 & 6 & 2 & 7 & 1 & 8 & 1 & 7\\ 
% DISTRICT & 7 & 2 & 4 & 3 & 1 & 10 & 1 & 6 & 1 & 5\\ 
% AWARD & 8 & 1 & 9 & 3 & 2 & 3 & 1 & 4 & 1 & 5\\ 
% DISEASE & 2 & 3 & 1 & 3 & 5 & 3 & 2 & 6 & 4 & 7\\ 
% PROFESSION & 5 & 1 & 5 & 5 & 1 & 3 & - & 5 & 1 & 6\\ 
% NUMBER & 1 & 3 & 3 & 2 & 2 & 6 & 2 & 2 & 1 & 5\\ 
% DATE & 3 & 1 & 2 & 1 & 5 & 2 & - & 2 & 6 & 1\\ 
% RELIGION & 1 & - & 5 & - & - & 1 & - & - & - & 3\\ 
% LANGUAGE & 2 & 2 & 3 & 2 & 2 & 2 & - & 2 & 1 & 4\\ 
% MONEY & 2 & - & 3 & 1 & - & - & - & 1 & - & 4\\ 
% ORDINAL & 2 & 2 & 1 & 1 & 2 & 6 & 1 & 1 & 1 & 2\\ 
% IDEOLOGY & 2 & 1 & 3 & 1 & 1 & 1 & - & - & - & 4\\ 
% TIME & - & - & 2 & - & 1 & 1 & - & 4 & 1 & 2\\ 
% PENALTY & 1 & 1 & 1 & 2 & 1 & 5 & 1 & 1 & 1 & 3\\ 
% AGE & 1 & - & 2 & 1 & - & 3 & - & 1 & - & 2\\ 
% CRIME & 2 & 3 & - & 1 & - & 1 & 1 & - & - & 1\\ 
% LAW & 1 & 1 & 2 & 2 & 1 & 2 & - & 2 & 1 & 1\\ 
% PERCENT & - & - & 1 & - & - & - & - & - & - & - \\
% \hline
% Total span matches & 4401 & 4732 & 4948 & 4853 & 3511 & 4283 & 2363 & 4618 & 2361 & 4595 \\
\bottomrule
\end{tabular}

\caption{Number of test instances with incorrectly recognized entity type. Top-16 entities cover approximately 85\% of all mismatches. The last row shows the number of correctly recognized spans for each system. Symbol `-' means that all system's predictions were correct. All calculations were performed for the \textit{full\_set} test set.}
\label{table:entity_mismatch}
\end{table}


